Entity Decomposition with Filtering: A Zero-Shot Clinical Named Entity Recognition Framework

Clinical named entity recognition (NER) aims to retrieve important entities within clinical narratives. Recent works have demonstrated that large language models (LLMs) can achieve strong performance in this task. While previous works focus on proprietary LLMs, we investigate how open NER LLMs, trained specifically for entity recognition, perform in clinical NER. Our initial experiment reveals significant contrast in performance for some clinical entities and how a simple exploitment on entity types can alleviate this issue. In this paper, we introduce a novel framework, entity decomposition with filtering, or EDF. Our key idea is to decompose the entity recognition task into several retrievals of entity sub-types and then filter them. Our experimental results demonstrate the efficacies of our framework and the improvements across all metrics, models, datasets, and entity types. Our analysis also reveals substantial improvement in recognizing previously missed entities using entity decomposition. We further provide a comprehensive evaluation of our framework and an in-depth error analysis to pave future works.

==> tables/table6.tex <==
\begin{table}[!t]
  \caption{Percentage (\%) of fully absent entities with and without and entity decomposer. A lower value is better.}
  \label{table_err_full_absent_ent}
  \centering
  \footnotesize
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}l@{\hspace{5pt}}
        @{\hspace{10pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{10pt}}
      }
      \toprule

      \multirow{2}{*}{Dataset} & \multirow{2}{*}{Entity Type} & \multicolumn{2}{c}{\makecell{Entity Decomposer}} \\
      \cmidrule{3-4}
      && \xmark & \cmark \\
      \midrule
      \multirow{3}{*}{i2b2 2010} & \texttt{Tr} & 28.7 & 5.5 \\
      & \texttt{Pr} & 19.9 & 8.1 \\
      & \texttt{Te} & 39.2 & 16.1 \\
      \midrule
      \multirow{4}{*}{i2b2 2012} & \texttt{Tr} & 30.5 & 9.5 \\
      & \texttt{Pr} & 21.4 & 9.9 \\
      & \texttt{Te} & 37.7 & 14.9 \\
      & \texttt{C-Dept} & 47.6 & 6.4 \\
      \midrule
      CLEF 2014 & \texttt{DD} & 58.8 & 29.2 \\
      \midrule
      \multirow{2}{*}{i2b2 2018} & \texttt{AD} & 54.0 & 16.5 \\
      & \texttt{ADE} & 68.6 & 26.4 \\
      
      \bottomrule
      \end{tabular}
  \end{threeparttable}
  \vskip -10pt
\end{table}

% \begin{table}[]
% \centering
% % \medium
% \small
% \caption{Percentage of fully absent entities with and without and entity decomposer}
% \vskip -10pt
% \tabcolsep 13pt
% \begin{tabular}{llcc}
% \hline
% \multirow{2}{*}{Dataset}   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Entity\\ Type\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Entity\\ Decomposer\end{tabular}} \\ \cline{3-4}
%                            &                                                                        & \xmark                                      & \cmark                                      \\ \hline
% \multirow{3}{*}{i2b2-2010} & \texttt{Tr}                                                                     & 28.7\%                                 & 5.5\%                                  \\
%                            & \texttt{Pr}                                                                     & 19.9\%                                 & 8.1\%                                  \\
%                            & \texttt{Te}                                                                     & 39.2\%                                 & 16.1\%                                 \\ \hline
% \multirow{4}{*}{i2b2-2012} & \texttt{Tr}                                                                     & 30.5\%                                 & 9.5\%                                  \\
%                            & \texttt{Pr}                                                                     & 21.4\%                                 & 9.9\%                                  \\
%                            & \texttt{Te}                                                                     & 37.7\%                                 & 14.9\%                                 \\
%                            & \texttt{C-Dept}                                                                 & 47.6\%                                 & 6.4\%                                  \\ \hline
% CLEF 2014                  & \texttt{DD}                                                                     & 58.8\%                                 & 29.2\%                                 \\ \hline
% \multirow{2}{*}{i2b2-2018} & \texttt{AD}                                                                     & 54.0\%                                 & 16.5\%                                 \\
%                            & \texttt{ADE}                                                                    & 68.6\%                                 & 26.4\%                                 \\ \hline
% \end{tabular}
% \label{table_err_full_absent_ent}
% \vskip -10pt
% \end{table}

==> tables/table_app4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\small
\vskip -10pt
\tabcolsep 11pt
\caption{Filter Prompt}
\begin{tabular}{llp{0.5\linewidth}}
\hline
Prompt Type                       & Entity Type         & Instruction                                                                                                                   \\ \hline
without Description (default)     &                     & Can '\{entity\}' be considered a/an \{entity\_type\}? Answer with yes or no.                                                            \\ \hline
\multirow{4}{*}{with Description} & Treatment           & Can '\{entity\}' be considered a procedure or substance given to a patient   to resolve a medical problem? Answer with yes or no. \\
                                  & Problem             & Can '\{entity\}' be considered an observation thought to be abnormal or   caused by a disease? Answer with yes or no.             \\
                                  & Test                & Can '\{entity\}' be considered a procedure or measure to find more   information about a medical problem? Answer with yes or no.  \\
                                  & Clinical Department & Can '\{entity\}' be considered a clinical unit or clinical service name?   Answer with yes or no.                                 \\ \hline
\end{tabular}
\label{table_app_filter_prompt}
\end{table*}
